Regret-Optimal Model-Free Reinforcement Learning for Discounted MDPs with Short Burn-In Time

A crucial problem in reinforcement learning is learning the optimal policy. We study this in tabular infinite-horizon discounted Markov decision processes under the online setting. The existing algorithms either fail to achieve regret optimality or have to incur a high memory and computational cost. In addition, existing optimal algorithms all require a long burn-in time in order to achieve optimal sample efficiency, i.e., their optimality is not guaranteed unless sample size surpasses a high threshold. We address both open problems by introducing a model-free algorithm that employs variance reduction and a novel technique that switches the execution policy in a slow-yet-adaptive manner. This is the first regret-optimal model-free algorithm in the discounted setting, with the additional benefit of a low burn-in time.

==> arxiv_chapters/algcopy.tex <==
%!TEX root = ../arxiv_main.tex

\section{Algorithm}\label{sec:alg}

\subsection{Q-Learning }

\paragraph{Q-learning with UCB}

\paragraph{Q-learning with UCB and reference advantage}

\subsection{Low-Switching}

\begin{algorithm}[t]
    \caption{Q-LowSwitching-Advantage \label{alg:main}}
        \textbf{Initialize:} For all $(s,a)$, $Q^{\mathrm{lazy}}(s,a), \overline{Q}(s,a), Q(s,a), Q^{\mathrm{UCB}}(s,a), Q^{\mathrm{R}}(s,a) \leftarrow \frac{1}{1-\gamma}$; $Q^{\mathrm{LCB}}(s,a) \leftarrow 0$; $N(s,a) \leftarrow 0$; $V(s) \leftarrow V^{\mathrm{R}}(s) = \frac{1}{1-\gamma}$; $\mu^{\mathrm{ref}}(s,a), \sigma^{\mathrm{ref}}(s,a), \mu^{\mathrm{adv}}(s,a), \sigma^{\mathrm{adv}}(s,a), \delta^{\mathrm{R}}(s,a), B^{\mathrm{R}}(s,a) \leftarrow 0$, $q(s,a) \leftarrow 0$; $M(s,a) \leftarrow 1$; $u^{\mathrm{ref}}(s) \leftarrow \mathrm{True}$; $H = \lceil\frac{2}{1-\gamma} \rceil$.
        
		\For{$t = 1, \cdots, T$}{
            Take action $a_t = \pi_{t}(s_t) = \arg \max_a Q^{\mathrm{lazy}}(s_t, a)$, and draw $s_{t+1} \sim P(\cdot | s_t, a_t)$.\\
            $N(s_t, a_t) \leftarrow N(s_t, a_t) + 1$; $n \leftarrow N(s_t, a_t)$.\\
		    $\eta_n \leftarrow \frac{H+1}{H+n}$.\\
		    $Q^{\mathrm{UCB}}(s_t, a_t) \leftarrow \textbf{update-ucb-q}()$.\\
		    $Q^{\mathrm{LCB}}(s_t, a_t) \leftarrow \textbf{update-lcb-q}()$.\\
		    $Q^{\mathrm{R}}(s_t, a_t) \leftarrow \textbf{update-ucb-q-advantage}()$.\\
		    $Q(s_t, a_t) \leftarrow \min \{Q^{\mathrm{R}}(s_t, a_t), Q^{\mathrm{UCB}}(s_t, a_t), Q(s_t, a_t)\}$.\\
		    $V(s_t) \leftarrow \max_a Q(s_t, a)$.\\
		    $V^{\mathrm{LCB}}(s_t) \leftarrow \max\{\max_a Q^{\mathrm{LCB}}(s_t, a), V^{\mathrm{LCB}}(s_t)\}$.\\
		    $q(s_t,a_t) \leftarrow q(s_t,a_t) + Q_{M(s_t, a_t)}(s_t, a_t) - Q(s_t, a_t)$.\\
            $Q^{\mathrm{lazy}} \leftarrow \overline{Q}$

            \If{$q(s_t,a_t) > \frac{1}{1-\gamma}$ \label{alg-line:q-cond}}{
                $M(s_t, a_t) \leftarrow t+1$;\\
                $\overline{Q} \leftarrow Q$;\\
		        $q(s_t,a_t) \leftarrow 0$;
            }

            \uIf{$V(s_{t}) - V^{\mathrm{LCB}}(s_{t}) > 3$ \label{alg-line:if-cond-1}}{
                $V^{\mathrm{R}}(s_{t}) \leftarrow V(s_{t})$, $u^{\mathrm{ref}}(s_{t}) = \mathrm{True}$; \label{alg-line:if-stat-1}
            }
            \ElseIf{$u^{\mathrm{ref}}(s_{t}) = \mathrm{True}$ \label{alg-line:elif-cond-1}}{
                $V^{\mathrm{R}}(s_{t}) \leftarrow V(s_{t})$, $u^{\mathrm{ref}}(s_{t}) = \mathrm{False}$. \label{alg-line:elif-stat-1}
            }

            \uIf{$V(s_{t+1}) - V^{\mathrm{LCB}}(s_{t+1}) > 3$ \label{alg-line:if-cond-2}}{
                $V^{\mathrm{R}}(s_{t+1}) \leftarrow V(s_{t+1})$, $u^{\mathrm{ref}}(s_{t+1}) = \mathrm{True}$; \label{alg-line:if-stat-2}
            }
            \ElseIf{$u^{\mathrm{ref}}(s_{t+1}) = \mathrm{True}$ \label{alg-line:elif-cond-2}}{
                $V^{\mathrm{R}}(s_{t+1}) \leftarrow V(s_{t+1})$, $u^{\mathrm{ref}}(s_{t+1}) = \mathrm{False}$. \label{alg-line:elif-stat-2}
            }
        }
\end{algorithm}

\begin{algorithm}[t]
    \caption{Auxiliary functions \label{alg:aux}}
    \SetKwFunction{FUCB}{update-ucb-q}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FUCB{}}{
        $Q^{\mathrm{UCB}}(s_t, a_t) \leftarrow (1 - \eta_n)Q^{\mathrm{UCB}}(s_t, a_t) + \eta_n\left(r(s_t, a_t) + \gamma V(s_{t+1}) + c_b\sqrt{\frac{\log\frac{SAT}{\delta}}{(1-\gamma)^3n}}\right).$ \label{alg-line:QUCB-update}
    }

    \SetKwFunction{FLCB}{update-ucb-q}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FLCB{}}{
        $Q^{\mathrm{LCB}}(s_t, a_t) \leftarrow (1 - \eta_n)Q^{\mathrm{LCB}}(s_t, a_t) + \eta_n\left(r(s_t, a_t) + \gamma V^{\mathrm{LCB}}(s_{t+1}) - c_b\sqrt{\frac{\log\frac{SAT}{\delta}}{(1-\gamma)^3n}}\right).$ \label{alg-line:QLCB-update}
    }

    \SetKwFunction{FUCBA}{update-ucb-q-advantage}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FUCBA{}}{
        $[\mu^{\mathrm{ref}}, \sigma^{\mathrm{ref}}](s_t, a_t) \leftarrow \textbf{update-moments}()$;
	
    	$[\delta^{\mathrm{R}}, B^{\mathrm{R}}](s_t, a_t) \leftarrow \textbf{update-bonus}()$;
    	
    	$b^{\mathrm{R}} \leftarrow B^{\mathrm{R}}(s_t, a_t) + (1 - \eta_n)\frac{\delta^{\mathrm{R}}(s_t, a_t)}{\eta_n} + c_b\frac{\log^2\frac{SAT}{\delta}}{n^{3/4}(1-\gamma)^2}$; \label{alg-line:b}
    	
    	$Q^{\mathrm{R}}(s_t, a_t) \leftarrow (1 - \eta_n)Q^{\mathrm{R}}(s_t, a_t) + \eta_n\left(r(s_t, a_t) + \gamma \left(V(s_{t+1}) - V^{\mathrm{R}}(s_{t+1}) + \mu^{\mathrm{ref}}(s_t, a_t)\right) + b^{\mathrm{R}}\right)$. \label{alg-line:QR-update}
    }

    \SetKwFunction{Fm}{update-moments}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\Fm{}}{
        $\mu^{\mathrm{ref}}(s_t, a_t) \leftarrow (1 - \frac{1}{n})\mu^{\mathrm{ref}}(s_t, a_t) + \frac{1}{n}V^{\mathrm{R}}(s_{t+1})$; \label{alg-line:mu-ref}
	
    	$\sigma^{\mathrm{ref}}(s_t, a_t) \leftarrow (1 - \frac{1}{n})\sigma^{\mathrm{ref}}(s_t, a_t) + \frac{1}{n}\left(V^{\mathrm{R}}(s_{t+1})\right)^2$; \label{alg-line:sigma-ref}
    	
    	$\mu^{\mathrm{adv}}(s_t, a_t) \leftarrow (1 - \eta_n)\mu^{\mathrm{adv}}(s_t, a_t) + \eta_n \left(V(s_{t+1}) - V^{\mathrm{R}}(s_{t+1})\right)$; \label{alg-line:mu-adv}
    	
    	$\sigma^{\mathrm{adv}}(s_t, a_t) \leftarrow (1 - \eta_n)\sigma^{\mathrm{adv}}(s_t, a_t) + \eta_n \left(V(s_{t+1}) - V^{\mathrm{R}}(s_{t+1})\right)^2$. \label{alg-line:sigma-adv}
    }

    \SetKwFunction{Fb}{update-bonus}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\Fb{}}{
        $B^{\mathrm{next}}(s_t, a_t) \leftarrow c_b\sqrt{\frac{\log\frac{SAT}{\delta}}{n}}\left(\sqrt{\sigma^{\mathrm{ref}}(s_t, a_t) - \left(\mu^{\mathrm{ref}}(s_t, a_t)\right)^2} + \frac{1}{\sqrt{1-\gamma}}\sqrt{\sigma^{\mathrm{adv}}(s_t, a_t) - \left(\mu^{\mathrm{adv}}(s_t, a_t)\right)^2}\right)$; \label{alg-line:Bnext}
	
    	$\delta^{\mathrm{R}}(s_t, a_t) \leftarrow B^{\mathrm{next}}(s_t, a_t) - B^{\mathrm{R}}(s_t, a_t)$; \label{alg-line:delta}
    	
    	$B^{\mathrm{R}}(s_t, a_t) \leftarrow B^{\mathrm{next}}(s_t, a_t)$. \label{alg-line:BR}
    }
\end{algorithm}

\begin{equation}
    \eta_n := \frac{\lceil\frac{2}{1-\gamma}\rceil + 1}{\lceil\frac{2}{1-\gamma}\rceil + n} \label{eq:learning-rate-def}
\end{equation}
